Near-infrared photometry of Galactic planetary nebulae with the VVV Survey

Planetary nebulae (PNe) are powerful tracers of evolved stellar populations. Among the 3000 known PNe in the Galaxy, about 600 are located within the 520 square-degree area covered by the VVV survey. The VVV photometric catalogue provides an important new dataset for the study of PNe, with high-resolution imaging in five near-infrared bands. Aperture photometry of known PNe in the VVV area was retrieved from source catalogues. Care was taken to minimise any confusion with field stars. The colours of the PNe we are determined for H-Ks, J-H, Z-Y, and Y-J, and compared to stars and to other types of emission line objects. Cloudy photo-ionisation models were used to predict colours for typical PNe. We present near-infrared photometry for 353 known PNe. The best separation from other objects is obtained in the H-Ks vs. J-H diagram. We calculated the emission-line contribution to the in-band flux based on a model for NGC 6720: we find that this is highest in the Z and Y bands at over 50%, lower in the J band at 40%, and lowest in the H and Ks bands at 20%. A new view of PNe in the wavelength domain of the Z and Y bands is shown. Photo-ionisation models are used to explore the observed colours in these bands. The Y band is shown to be dominated by HeI 1.083 mu and HeII 1.012 mu, and colours involving this band are very sensitive to the temperature of the ionizing star. The VVV survey represents a unique dataset for studing crowded and obscured regions in the Galactic plane. The diagnostic diagrams presented here allow one to study the properties of known PNe and to uncover objects not previously classified.

==> cds/ReadMe.tex <==
J/A+A/vol/page     Planetary nebulae with VVV     (Weidmann+, 2013)
================================================================================
Near-infrared photometry of Galactic planetary nebulae with the
VVV Survey
W. A. Weidmann, R. Gamen, P.A.M. van Hoof, A. Zijlstra, D. Minniti and M. G. Volpe
    <Astron. Astrophys. vol, page (2013)>
    =2013A&A...VVV.ppppI     (SIMBAD/NED BibCode)
================================================================================
Keywords: planetary nebulae: general – infrared: ISM – catalogues


Description:
Aperture photometry of known PNe in the VVV  area was retrieved 
from source catalogues. 
579 PNe were selected from the VVV (VISTA Variables
in the Via Lactea) survey catalogue.
Of these 353 present near-infrared photometry,
75 are highly extended sources, and 123
PNe could not be related to any source in the VVV images, the remainder 
are sources which NIR emission of the PN is detected in the frames, 
but there are no photometric data in the VSA database.



File Summary:
--------------------------------------------------------------------------------
  FileName   Lrecl  Records   Explanations
--------------------------------------------------------------------------------
ReadMe          80        .   This file
table3.dat   (len)   (rows)   NIR photometry catalogue of PNe
--------------------------------------------------------------------------------

Byte-by-byte Description of file: table1.dat
--------------------------------------------------------------------------------
   Bytes Format Units   Label     Explanations
--------------------------------------------------------------------------------
   1- 12   A12   ---     name      Main designation
      13   A1    ---     note      (N/*) new NIR determination/probable not central star
  15- 25   A10   ---     PN G      Designation of the Galactic Planetary Nebula
  27- 28   I2    h       RAh       Right ascension (J2000)
  30- 31   I2    min     RAm       Right ascension (J2000)
  33- 36   F4.2  s       RAs       Right ascension (J2000)
      38   A1    ---     DE-       Declination sign
  39- 40   I2    deg     DEd       Declination (J2000)
  42- 43   I2    arcmin  DEm       Declination (J2000)
  45- 46   I2    arcsec  DEs       Declination (J2000)
  48- 49   A2    ---     type      Source class (Note 1)
  51- 55   F5.2  mag     Z         VVV Z band magnitude
      57   A1    ---     f_Z       VVV photometry flag (Note 2)
  59- 62   F4.1  mag     e_Z       VVV Z band magnitude error
  64- 68   F5.2  mag     Y         VVV Y band magnitude
      70   A1    ---     f_Y       VVV photometry flag (Note 2)
  72- 75   F4.1  mag     e_Y       VVV Y band magnitude error
  77- 81   F5.2  mag     J         VVV J band magnitude
      83   A1    ---     f_J       VVV photometry flag (Note 2)
  85- 88   F4.1  mag     e_J       VVV J band magnitude error
  90- 94   F5.2  mag     H         VVV H band magnitude
      96   A1    ---     f_H       VVV photometry flag (Note 2)
  98- 101  F4.1  mag     e_H       VVV H band magnitude error
 103- 107  F5.2  mag     Ks        VVV Ks band magnitude
      109  A1    ---     f_Ks      VVV photometry flag (Note 2)
 111- 114  F4.1  mag     e_Ks      VVV Ks band magnitude error



cuidado con las magnitudes de un digito

--------------------------------------------------------------------------------
Note (1): 
“-1” is used to denote stellar objects, “-2” borderline stellar and “1” is used for non-stellar objects.


Note (2)
Flag indicating that the magnitude is near the saturation limits.

--------------------------------------------------------------------------------

References:
  The addition of the "BibCode" (a 19-digit such as 1994A&AS..103..135A
  used by SIMBAD, NED, and ADS Abstract Services) would help to generate
  links to the appropriate papers.
================================================================================
(End)          Name [Institution]                                    01-Jan-2003






















==> cds/table-4.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\longtabL{4}{
\begin{landscape}
\begin{longtable}{lcccccccccc}
\caption{\label{tablita-3} Petrosian radius of the 353 PNe listed in Table~\ref{tablita}.
When $\sigma$=0 means that $\sigma$$<0.05$ and when $\sigma$$\equiv n$ 
means that there is only one measured so it is not possible to give
an stdev.}\\
\hline\hline
name & P$_Z$ & $\sigma$ & P$_Y$ & $\sigma$ & P$_J$ & $\sigma$ & P$_H$ & $\sigma$ & P$_{Ks}$ & $\sigma$ \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
name & P$_Z$ & $\sigma$ & P$_Y$ & $\sigma$ & P$_J$ & $\sigma$ & P$_H$ & $\sigma$ & P$_{Ks}$ & $\sigma$ \\
\hline
\endhead
\hline
\endfoot
%%
Ae 1  &  -  &  -  &  -  &  -  &  2.2  &  0.7  &  1.2  &  0.1  &  1.5  &  0.2  \\
Ae 2-E  &  3.0  &  1.2  &  2.9  &  0.4  &  -  &  -  &  -  &  -  &  -  &  -  \\
Ae 2-F  &  2.8  &  0.8  &  1.7  &  0.1  &  1.7  &  n  &  -  &  -  &  1.8  &  n  \\
Ae 2-G  &  1.7  &  0.2  &  1.6  &  0.0  &  -  &  -  &  -  &  -  &  -  &  -  \\
Ae 2-H  &  -  &  -  &  -  &  -  &  2.2  &  n  &  1.7  &  n  &  1.7  &  0.1  \\
Ae 2-I  &  3.2  &  0.0  &  3.1  &  0.1  &  -  &  -  &  -  &  -  &  -  &  -  \\
Ae 2-J  &  2.9  &  0.0  &  2.5  &  0.0  &  -  &  -  &  -  &  -  &  -  &  -  \\
Ae 2-K  &  -  &  -  &  3.3  &  0.0  &  -  &  -  &  -  &  -  &  -  &  -  \\
Ae 2-R  &  1.8  &  0.2  &  2.0  &  0.0  &  2.0  &  0.2  &  2.5  &  0.3  &  2.2  &  0.3  \\
BeVa 1  &  2.1  &  0.0  &  2.1  &  0.0  &  1.7  &  0.0  &  1.7  &  0.0  &  1.9  &  0.1  \\
Bl 3-13  &  3.3  &  0.4  &  2.6  &  0.5  &  2.9  &  0.3  &  2.4  &  n  &  2.4  &  0.2  \\
BMP1522-5729  &  3.3  &  0.4  &  3.3  &  0.4  &  3.3  &  0.7  &  3.6  &  0.1  &  3.3  &  0.3  \\
BMP1524-5746  &  2.2  &  0.0  &  2.1  &  0.0  &  2.0  &  0.0  &  2.0  &  0.0  &  2.1  &  0.0  \\
BMP1622-5144  &  1.8  &  0.1  &  1.8  &  0.1  &  1.5  &  0.2  &  1.6  &  0.3  &  1.5  &  0.2  \\
Cn 2-1  &  -  &  -  &  -  &  -  &  2.0  &  0.0  &  1.9  &  0.0  &  1.9  &  0.1  \\
H 1-8  &  3.3  &  0.0  &  3.1  &  0.0  &  -  &  -  &  -  &  -  &  -  &  -  \\
H 1-9  &  2.6  &  0.5  &  2.6  &  0.3  &  2.8  &  0.1  &  2.3  &  0.0  &  2.0  &  0.1  \\
H 1-16  &  -  &  -  &  -  &  -  &  2.3  &  0.0  &  2.2  &  0.1  &  2.2  &  0.1  \\
H 1-17  &  2.6  &  0.3  &  2.3  &  0.1  &  2.6  &  0.3  &  1.8  &  0.1  &  1.5  &  0.0  \\
H 1-18  &  2.3  &  0.1  &  2.1  &  0.0  &  -  &  -  &  -  &  -  &  1.9  &  0.0  \\
H 1-19  &  1.6  &  0.0  &  1.3  &  0.1  &  -  &  -  &  -  &  -  &  -  &  -  \\
H 1-20  &  3.0  &  0.0  &  2.9  &  0.0  &  -  &  -  &  -  &  -  &  -  &  -  \\
H 1-22  &  -  &  -  &  -  &  -  &  3.0  &  0.0  &  3.1  &  0.2  &  2.9  &  0.0  \\
H 1-23  &  2.4  &  0.0  &  2.3  &  0.0  &  2.3  &  0.0  &  2.2  &  0.0  &  2.3  &  0.0  \\
H 1-29  &  2.4  &  0.0  &  2.4  &  0.0  &  2.4  &  0.1  &  2.2  &  0.1  &  2.1  &  0.1  \\
H 1-30  &  -  &  -  &  -  &  -  &  2.4  &  0.0  &  2.0  &  0.0  &  2.1  &  0.1  \\
H 1-32  &  2.4  &  0.6  &  1.7  &  0.0  &  1.6  &  0.1  &  1.4  &  0.0  &  1.4  &  0.0  \\
H 1-33  &  2.5  &  0.2  &  2.4  &  0.2  &  2.2  &  0.0  &  2.1  &  0.1  &  2.1  &  0.0  \\
H 1-34  &  2.0  &  0.0  &  1.9  &  0.0  &  1.6  &  0.0  &  1.6  &  0.0  &  1.5  &  0.1  \\
H 1-35  &  2.3  &  0.0  &  2.1  &  0.0  &  1.8  &  0.1  &  1.6  &  0.0  &  1.6  &  0.0  \\
H 1-39  &  -  &  -  &  -  &  -  &  2.0  &  0.1  &  1.7  &  0.0  &  1.9  &  0.1  \\
H 1-40  &  2.2  &  0.1  &  2.1  &  0.1  &  1.7  &  0.0  &  1.6  &  0.1  &  1.6  &  0.1  \\
H 1-41  &  -  &  -  &  -  &  -  &  4.3  &  0.6  &  3.6  &  0.3  &  4.7  &  0.8  \\
H 1-43  &  -  &  -  &  -  &  -  &  1.6  &  0.0  &  1.5  &  0.1  &  1.6  &  0.1  \\
H 1-44  &  -  &  -  &  -  &  -  &  2.8  &  0.1  &  3.2  &  0.4  &  3.2  &  0.3  \\
H 1-46  &  -  &  -  &  -  &  -  &  1.8  &  0.3  &  2.0  &  0.7  &  1.6  &  0.2  \\
H 1-54  &  -  &  -  &  -  &  -  &  1.5  &  0.0  &  1.5  &  0.1  &  1.5  &  0.1  \\
H 1-55  &  -  &  -  &  -  &  -  &  2.1  &  0.0  &  2.2  &  0.1  &  2.3  &  0.1  \\
H 1-56  &  -  &  -  &  -  &  -  &  2.6  &  0.0  &  2.6  &  0.0  &  2.6  &  0.0  \\
H 1-58  &  1.9  &  0.1  &  1.6  &  0.0  &  1.2  &  0.1  &  1.1  &  0.0  &  1.2  &  0.0  \\
H 1-59  &  -  &  -  &  -  &  -  &  1.3  &  0.1  &  1.2  &  0.1  &  1.2  &  0.1  \\
H 1-60  &  -  &  -  &  -  &  -  &  2.2  &  0.1  &  1.8  &  0.2  &  1.5  &  0.2  \\
H 1-61  &  2.2  &  0.1  &  2.2  &  0.1  &  1.8  &  0.1  &  1.6  &  0.1  &  1.5  &  0.1  \\
H 1-62  &  -  &  -  &  -  &  -  &  2.5  &  0.2  &  2.3  &  0.1  &  2.4  &  0.2  \\
H 1-63  &  -  &  -  &  -  &  -  &  1.4  &  0.1  &  1.2  &  0.1  &  1.2  &  0.1  \\
H 1-64  &  2.7  &  0.2  &  2.8  &  0.4  &  2.7  &  0.0  &  2.5  &  0.2  &  2.4  &  0.2  \\
H 1-66  &  -  &  -  &  -  &  -  &  -  &  -  &  1.7  &  0.2  &  -  &  -  \\
H 2-1  &  -  &  -  &  -  &  -  &  2.4  &  0.1  &  2.0  &  0.2  &  2.0  &  0.1  \\
H 2-10  &  2.7  &  0.1  &  2.6  &  0.1  &  2.5  &  0.0  &  2.3  &  0.0  &  2.2  &  0.0  \\
H 2-13  &  4.6  &  0.3  &  4.4  &  0.6  &  3.1  &  0.3  &  3.0  &  0.1  &  2.7  &  0.5  \\
H 2-20  &  -  &  -  &  -  &  -  &  2.2  &  0.0  &  2.0  &  0.0  &  2.2  &  0.0  \\
H 2-23  &  3.5  &  0.2  &  2.8  &  0.9  &  2.0  &  0.9  &  1.3  &  0.1  &  1.7  &  0.6  \\
H 2-24  &  2.4  &  1.3  &  2.1  &  1.0  &  1.5  &  0.0  &  2.2  &  0.2  &  3.6  &  0.3  \\
H 2-25  &  2.3  &  0.0  &  2.0  &  0.0  &  1.9  &  0.0  &  1.8  &  0.0  &  2.2  &  0.0  \\
H 2-26  &  1.6  &  n  &  -  &  -  &  -  &  -  &  1.2  &  n  &  1.3  &  0.1  \\
H 2-27  &  3.0  &  0.0  &  2.5  &  0.0  &  2.0  &  0.1  &  1.4  &  0.1  &  2.0  &  0.1  \\
H 2-29  &  1.3  &  n  &  1.0  &  0.1  &  0.9  &  n  &  -  &  -  &  -  &  -  \\
H 2-35  &  -  &  -  &  -  &  -  &  1.3  &  0.2  &  0.9  &  n  &  -  &  -  \\
H 2-36  &  -  &  -  &  -  &  -  &  1.4  &  0.4  &  1.0  &  0.1  &  -  &  -  \\
H 2-37  &  2.8  &  0.1  &  2.4  &  0.2  &  2.7  &  0.1  &  1.5  &  0.3  &  2.4  &  0.4  \\
H 2-39  &  -  &  -  &  -  &  -  &  2.0  &  0.6  &  1.3  &  0.1  &  2.4  &  0.6  \\
H 2-40  &  -  &  -  &  -  &  -  &  2.1  &  0.0  &  1.8  &  0.0  &  1.8  &  0.0  \\
H 2-41  &  -  &  -  &  -  &  -  &  -  &  -  &  1.2  &  0.1  &  1.2  &  0.2  \\
H 2-42  &  -  &  -  &  -  &  -  &  2.6  &  0.0  &  2.5  &  0.0  &  2.4  &  0.3  \\
H 2-45  &  2.2  &  0.0  &  2.2  &  0.0  &  2.2  &  0.0  &  2.1  &  0.0  &  2.2  &  0.0  \\
H 2-46  &  2.8  &  0.2  &  2.9  &  0.2  &  2.6  &  0.1  &  2.3  &  0.1  &  1.8  &  0.1  \\
Hb 5  &  -  &  -  &  -  &  -  &  5.0  &  0.3  &  4.2  &  0.4  &  4.0  &  0.2  \\
He 2-84  &  3.3  &  0.4  &  2.7  &  0.0  &  2.6  &  0.0  &  2.5  &  0.1  &  2.7  &  0.3  \\
He 2-90  &  3.4  &  0.3  &  2.7  &  0.3  &  3.2  &  0.4  &  3.2  &  0.1  &  3.3  &  0.5  \\
He 2-96  &  2.4  &  0.1  &  2.4  &  0.0  &  2.3  &  0.0  &  2.1  &  0.0  &  2.2  &  0.1  \\
He 2-106  &  2.4  &  0.3  &  3.2  &  0.6  &  5.6  &  0.8  &  7.9  &  n  &  8.4  &  1.9  \\
He 2-117  &  4.1  &  0.0  &  4.1  &  0.1  &  4.1  &  0.0  &  3.9  &  0.0  &  3.9  &  0.1  \\
He 2-133  &  3.8  &  0.3  &  3.8  &  0.2  &  3.4  &  0.0  &  3.3  &  0.0  &  3.2  &  0.0  \\
He 2-140  &  3.2  &  0.0  &  3.1  &  0.0  &  3.1  &  0.1  &  3.0  &  0.0  &  3.1  &  0.1  \\
He 2-142  &  4.5  &  0.1  &  4.3  &  0.3  &  4.5  &  0.0  &  3.7  &  0.6  &  3.9  &  0.9  \\
He 2-143  &  2.8  &  0.0  &  2.8  &  0.1  &  2.5  &  0.0  &  2.3  &  0.0  &  2.4  &  0.1  \\
He 2-153  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  1.1  &  n  \\
He 2-250  &  4.2  &  0.0  &  3.9  &  0.1  &  3.9  &  0.0  &  3.7  &  n  &  4.0  &  0.2  \\
He 2-262  &  3.7  &  0.2  &  3.9  &  0.0  &  2.9  &  0.6  &  3.6  &  0.4  &  3.1  &  0.7  \\
Hf 2-1  &  -  &  -  &  -  &  -  &  2.6  &  0.1  &  1.8  &  0.6  &  2.3  &  0.4  \\
Hf 2-2  &  1.7  &  0.1  &  1.4  &  0.1  &  1.3  &  0.1  &  0.9  &  0.1  &  1.0  &  0.1  \\
IC 4673  &  3.3  &  0.1  &  3.1  &  0.1  &  2.2  &  0.8  &  2.1  &  0.1  &  -  &  -  \\
IRAS18023-2513  &  2.6  &  0.4  &  3.3  &  0.2  &  3.5  &  0.8  &  3.2  &  0.2  &  4.3  &  0.5  \\
JaFu 1  &  -  &  -  &  -  &  -  &  2.1  &  0.1  &  1.7  &  0.4  &  1.8  &  0.1  \\
JaSt 2  &  -  &  -  &  1.5  &  n  &  -  &  -  &  -  &  -  &  -  &  -  \\
JaSt 8  &  -  &  -  &  -  &  -  &  1.1  &  0.1  &  0.9  &  0.1  &  0.9  &  0.0  \\
JaSt 16  &  -  &  -  &  -  &  -  &  3.0  &  0.1  &  2.6  &  0.1  &  2.5  &  0.6  \\
JaSt 36  &  -  &  -  &  -  &  -  &  2.5  &  0.0  &  2.3  &  0.0  &  2.5  &  0.1  \\
JaSt 46  &  -  &  -  &  -  &  -  &  2.5  &  0.0  &  2.3  &  0.4  &  2.5  &  0.0  \\
JaSt 52  &  -  &  -  &  -  &  -  &  1.6  &  0.1  &  1.5  &  0.1  &  1.5  &  0.1  \\
JaSt 54  &  -  &  -  &  -  &  -  &  1.4  &  0.1  &  1.8  &  0.3  &  2.4  &  0.2  \\
JaSt 56  &  -  &  -  &  -  &  -  &  2.4  &  0.1  &  2.1  &  0.1  &  2.2  &  0.1  \\
JaSt 63  &  -  &  -  &  -  &  -  &  0.9  &  n  &  2.8  &  0.0  &  -  &  -  \\
JaSt 64  &  1.7  &  0.0  &  1.7  &  0.0  &  1.7  &  0.0  &  1.5  &  0.0  &  1.6  &  0.1  \\
JaSt 65  &  2.4  &  0.5  &  2.4  &  0.2  &  2.5  &  0.7  &  2.0  &  0.1  &  2.1  &  0.4  \\
JaSt 69  &  -  &  -  &  -  &  -  &  1.1  &  0.1  &  1.1  &  0.2  &  1.0  &  0.1  \\
JaSt 71  &  -  &  -  &  -  &  -  &  2.0  &  0.0  &  1.9  &  0.0  &  2.0  &  0.0  \\
JaSt 74  &  -  &  -  &  -  &  -  &  2.5  &  0.2  &  2.4  &  0.0  &  2.5  &  0.1  \\
JaSt 75  &  -  &  -  &  -  &  -  &  2.0  &  0.1  &  1.9  &  0.1  &  1.9  &  0.2  \\
JaSt 78  &  -  &  -  &  -  &  -  &  1.2  &  0.1  &  1.1  &  0.1  &  1.5  &  0.3  \\
JaSt 79  &  1.8  &  0.1  &  1.7  &  0.1  &  1.8  &  0.3  &  2.9  &  0.8  &  3.0  &  1.1  \\
JaSt 81  &  -  &  -  &  -  &  -  &  1.9  &  0.1  &  1.8  &  0.0  &  1.8  &  0.3  \\
JaSt 95  &  -  &  -  &  -  &  -  &  1.1  &  0.0  &  1.1  &  0.1  &  1.3  &  0.2  \\
K 5-5  &  2.3  &  0.6  &  2.0  &  0.1  &  1.6  &  0.0  &  1.5  &  0.0  &  1.5  &  0.0  \\
K 5-6  &  -  &  -  &  -  &  -  &  2.1  &  0.2  &  2.5  &  0.4  &  2.4  &  0.3  \\
K 5-8  &  1.8  &  0.1  &  1.7  &  0.0  &  1.8  &  0.1  &  2.2  &  0.2  &  1.7  &  0.6  \\
K 5-10  &  1.9  &  0.5  &  2.0  &  0.3  &  1.9  &  0.3  &  2.3  &  0.3  &  1.1  &  0.1  \\
K 5-18  &  -  &  -  &  -  &  -  &  1.0  &  0.1  &  -  &  -  &  -  &  -  \\
K 5-19  &  2.5  &  0.0  &  -  &  -  &  -  &  -  &  1.7  &  0.2  &  2.2  &  0.3  \\
K 5-20  &  3.0  &  0.4  &  2.7  &  0.1  &  2.5  &  0.0  &  2.1  &  0.1  &  2.9  &  0.3  \\
K 6-7  &  2.9  &  n  &  2.8  &  n  &  2.2  &  0.4  &  1.6  &  0.3  &  1.7  &  0.5  \\
KnFs 11  &  -  &  -  &  -  &  -  &  2.0  &  0.6  &  1.6  &  0.1  &  2.5  &  0.5  \\
KnFs 12  &  -  &  -  &  -  &  -  &  1.7  &  0.0  &  1.3  &  0.0  &  2.0  &  0.9  \\
KnFs 13  &  1.2  &  0.1  &  1.3  &  0.1  &  1.1  &  0.1  &  0.9  &  n  &  -  &  -  \\
KnFs 14  &  -  &  -  &  -  &  -  &  1.1  &  0.0  &  1.2  &  0.1  &  1.1  &  0.1  \\
KnFs 16  &  -  &  -  &  -  &  -  &  1.4  &  0.2  &  1.3  &  0.1  &  1.4  &  0.2  \\
KnFs 19  &  -  &  -  &  -  &  -  &  1.8  &  0.3  &  1.4  &  0.4  &  0.9  &  n  \\
Lo 10  &  -  &  -  &  -  &  -  &  -  &  -  &  1.1  &  0.0  &  1.5  &  0.5  \\
M 1-19  &  -  &  -  &  -  &  -  &  2.7  &  0.0  &  2.5  &  0.0  &  2.6  &  0.1  \\
M 1-26  &  -  &  -  &  -  &  -  &  3.3  &  0.5  &  3.0  &  0.4  &  3.0  &  0.3  \\
M 1-28  &  -  &  -  &  -  &  -  &  0.9  &  n  &  -  &  -  &  1.0  &  n  \\
M 1-30  &  -  &  -  &  -  &  -  &  3.3  &  0.0  &  3.2  &  0.0  &  3.2  &  0.1  \\
M 1-31  &  -  &  -  &  -  &  -  &  2.3  &  0.0  &  2.3  &  0.1  &  2.3  &  0.1  \\
M 1-34  &  -  &  -  &  -  &  -  &  -  &  -  &  2.2  &  n  &  2.0  &  n  \\
M 1-37  &  2.6  &  0.1  &  2.4  &  0.0  &  2.6  &  0.2  &  2.5  &  0.2  &  2.5  &  0.3  \\
M 1-38  &  2.5  &  0.0  &  2.5  &  0.2  &  2.8  &  0.4  &  1.8  &  0.4  &  2.3  &  0.3  \\
M 2-10  &  -  &  -  &  -  &  -  &  2.5  &  0.0  &  2.2  &  0.0  &  2.5  &  0.1  \\
M 2-11  &  -  &  -  &  -  &  -  &  2.9  &  0.6  &  1.7  &  0.1  &  2.1  &  0.3  \\
M 2-14  &  3.1  &  0.4  &  3.0  &  0.4  &  2.3  &  0.0  &  2.1  &  0.0  &  2.1  &  0.0  \\
M 2-16  &  3.1  &  0.1  &  2.9  &  0.1  &  2.8  &  0.1  &  2.6  &  0.1  &  2.5  &  0.1  \\
M 2-18  &  2.3  &  0.2  &  2.4  &  0.5  &  2.3  &  0.4  &  2.0  &  0.1  &  2.0  &  0.1  \\
M 2-19  &  -  &  -  &  -  &  -  &  1.5  &  0.1  &  1.3  &  0.1  &  1.4  &  0.2  \\
M 2-21  &  2.4  &  0.0  &  2.3  &  0.0  &  4.5  &  0.0  &  2.4  &  0.0  &  2.9  &  0.5  \\
M 2-22  &  -  &  -  &  -  &  -  &  3.6  &  0.9  &  2.5  &  1.6  &  2.9  &  1.2  \\
M 2-23  &  2.4  &  0.3  &  2.0  &  0.2  &  2.1  &  0.2  &  2.0  &  0.4  &  1.9  &  0.5  \\
M 2-24  &  -  &  -  &  -  &  -  &  1.9  &  0.0  &  1.9  &  0.0  &  2.4  &  0.1  \\
M 2-25  &  -  &  -  &  -  &  -  &  1.6  &  0.4  &  -  &  -  &  -  &  -  \\
M 2-26  &  2.0  &  0.0  &  2.2  &  0.1  &  1.6  &  0.3  &  1.0  &  0.1  &  1.1  &  0.1  \\
M 2-27  &  -  &  -  &  -  &  -  &  2.3  &  0.1  &  2.2  &  0.1  &  2.2  &  0.1  \\
M 2-28  &  3.0  &  0.0  &  2.6  &  0.0  &  3.0  &  0.1  &  1.9  &  0.0  &  2.0  &  0.3  \\
M 2-30  &  -  &  -  &  -  &  -  &  2.7  &  0.0  &  2.7  &  0.0  &  2.6  &  0.0  \\
M 2-31  &  3.2  &  0.0  &  3.2  &  0.1  &  3.1  &  0.0  &  3.0  &  0.0  &  2.9  &  0.0  \\
M 2-32  &  -  &  -  &  -  &  -  &  2.8  &  0.2  &  2.6  &  0.2  &  2.7  &  0.1  \\
M 2-33  &  -  &  -  &  -  &  -  &  2.9  &  0.0  &  2.9  &  0.0  &  3.1  &  0.1  \\
M 2-34  &  1.4  &  0.0  &  1.3  &  0.0  &  1.3  &  0.0  &  1.3  &  0.0  &  1.3  &  0.0  \\
M 2-36  &  -  &  -  &  -  &  -  &  3.9  &  0.4  &  3.1  &  0.3  &  3.3  &  0.3  \\
M 2-37  &  -  &  -  &  -  &  -  &  1.9  &  0.1  &  1.7  &  0.1  &  2.2  &  0.8  \\
M 2-38  &  -  &  -  &  -  &  -  &  -  &  -  &  1.3  &  0.2  &  -  &  -  \\
M 2-39  &  -  &  -  &  -  &  -  &  2.2  &  0.2  &  1.6  &  0.3  &  1.5  &  0.1  \\
M 2-41  &  1.6  &  0.4  &  1.6  &  0.7  &  1.1  &  0.0  &  2.0  &  0.7  &  1.1  &  n  \\
M 2-42  &  -  &  -  &  -  &  -  &  3.4  &  0.1  &  3.3  &  0.2  &  3.3  &  0.1  \\
M 3-7  &  4.1  &  1.4  &  2.1  &  0.0  &  2.1  &  n  &  -  &  -  &  2.6  &  1.3  \\
M 3-10  &  3.4  &  0.2  &  3.3  &  0.1  &  3.3  &  0.1  &  2.6  &  0.2  &  2.4  &  0.0  \\
M 3-14  &  4.6  &  0.0  &  4.2  &  0.6  &  4.7  &  0.0  &  3.2  &  0.3  &  3.7  &  0.9  \\
M 3-16  &  3.4  &  0.3  &  3.2  &  0.3  &  3.2  &  0.1  &  2.9  &  0.4  &  2.9  &  0.3  \\
M 3-17  &  2.6  &  0.1  &  2.3  &  0.0  &  2.3  &  0.0  &  2.1  &  0.1  &  2.3  &  0.0  \\
M 3-19  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  2.7  &  n  \\
M 3-20  &  2.9  &  0.0  &  2.8  &  0.0  &  2.5  &  0.0  &  2.5  &  0.0  &  2.5  &  0.1  \\
M 3-22  &  -  &  -  &  -  &  -  &  2.7  &  n  &  1.6  &  n  &  1.9  &  0.4  \\
M 3-26  &  -  &  -  &  -  &  -  &  1.3  &  0.3  &  1.1  &  0.0  &  1.0  &  n  \\
M 3-38  &  -  &  -  &  -  &  -  &  1.9  &  0.2  &  1.6  &  0.0  &  1.6  &  0.0  \\
M 3-41  &  3.2  &  0.3  &  3.0  &  0.2  &  3.2  &  0.1  &  2.3  &  0.6  &  2.2  &  0.5  \\
M 3-42  &  5.3  &  1.1  &  2.0  &  n  &  -  &  -  &  -  &  -  &  1.4  &  0.4  \\
M 3-43  &  -  &  -  &  -  &  -  &  3.2  &  0.3  &  3.2  &  0.3  &  3.2  &  0.3  \\
M 3-45  &  3.3  &  0.8  &  3.5  &  0.5  &  3.5  &  0.1  &  2.3  &  0.2  &  2.7  &  0.2  \\
M 3-46  &  1.9  &  0.3  &  1.5  &  0.3  &  1.9  &  0.2  &  1.2  &  n  &  1.5  &  0.1  \\
M 3-51  &  -  &  -  &  -  &  -  &  1.6  &  0.1  &  1.8  &  0.1  &  1.6  &  0.3  \\
M 4-6  &  3.3  &  0.5  &  2.6  &  0.0  &  -  &  -  &  -  &  -  &  2.8  &  0.4  \\
M 4-7  &  4.2  &  0.8  &  3.3  &  0.9  &  4.0  &  1.4  &  2.8  &  0.5  &  4.3  &  1.4  \\
MaC 1-11  &  2.8  &  0.2  &  2.9  &  0.2  &  2.6  &  0.1  &  2.6  &  0.2  &  2.5  &  0.1  \\
MPA1157-6226  &  1.5  &  0.1  &  2.8  &  0.2  &  2.8  &  0.4  &  3.6  &  0.6  &  2.8  &  0.9  \\
MPA1221-6413  &  2.5  &  0.0  &  2.2  &  0.0  &  2.4  &  0.0  &  2.2  &  0.0  &  2.2  &  0.1  \\
MPA1235-6318  &  3.7  &  0.5  &  3.3  &  0.3  &  3.6  &  0.1  &  3.1  &  0.5  &  3.5  &  0.5  \\
MPA1242-6459  &  2.6  &  0.2  &  2.6  &  0.4  &  2.4  &  0.0  &  2.3  &  0.0  &  2.3  &  0.0  \\
MPA1243-6428  &  2.6  &  0.0  &  2.5  &  0.0  &  2.3  &  0.1  &  2.0  &  0.1  &  1.8  &  0.1  \\
MPA1249-6414  &  1.8  &  0.1  &  2.0  &  0.1  &  1.9  &  0.1  &  1.7  &  0.1  &  1.9  &  0.2  \\
MPA1309-6415  &  2.9  &  0.0  &  2.7  &  0.5  &  2.2  &  0.6  &  1.9  &  0.8  &  2.8  &  0.6  \\
MPA1319-6418  &  1.9  &  0.0  &  1.9  &  0.0  &  1.9  &  0.0  &  1.9  &  0.0  &  2.2  &  0.3  \\
MPA1326-6407  &  1.6  &  0.9  &  2.0  &  0.7  &  2.3  &  0.8  &  2.4  &  n  &  2.0  &  1.1  \\
MPA1327-6031  &  1.8  &  n  &  1.8  &  n  &  1.7  &  n  &  1.9  &  n  &  1.7  &  0.1  \\
MPA1346-6418  &  3.7  &  n  &  3.7  &  0.7  &  3.8  &  0.2  &  3.0  &  0.5  &  2.4  &  1.5  \\
MPA1354-6337  &  3.6  &  0.0  &  3.5  &  0.0  &  3.4  &  0.1  &  3.4  &  0.1  &  3.2  &  0.3  \\
MPA1428-6234  &  1.7  &  0.1  &  1.6  &  0.0  &  2.0  &  0.5  &  2.1  &  0.5  &  2.6  &  0.5  \\
MPA1430-6251  &  2.7  &  0.3  &  3.1  &  0.3  &  3.3  &  0.3  &  2.8  &  0.3  &  3.0  &  0.9  \\
MPA1439-5816  &  2.2  &  0.1  &  2.1  &  0.2  &  1.6  &  0.1  &  1.5  &  0.2  &  1.5  &  0.2  \\
MPA1441-6114  &  3.4  &  0.6  &  2.9  &  0.0  &  2.8  &  0.0  &  2.7  &  0.1  &  2.7  &  0.1  \\
MPA1517-5538  &  -  &  -  &  -  &  -  &  1.0  &  0.1  &  1.1  &  0.1  &  1.1  &  0.1  \\
MPA1520-5517  &  1.2  &  n  &  1.4  &  n  &  3.4  &  n  &  1.7  &  n  &  2.2  &  0.9  \\
MPA1522-5917  &  2.9  &  0.1  &  2.7  &  0.6  &  3.0  &  0.3  &  3.1  &  0.4  &  2.7  &  0.1  \\
MPA1523-5710  &  5.3  &  n  &  3.9  &  1.9  &  3.1  &  1.0  &  2.7  &  0.5  &  3.7  &  1.1  \\
MPA1530-5801  &  2.8  &  0.0  &  2.8  &  0.2  &  2.8  &  0.1  &  2.6  &  0.4  &  2.8  &  0.3  \\
MPA1605-5319  &  3.0  &  0.1  &  3.0  &  0.1  &  3.1  &  0.2  &  3.0  &  0.3  &  2.8  &  0.1  \\
MPA1606-5407  &  2.3  &  0.1  &  2.1  &  0.1  &  1.9  &  0.2  &  1.6  &  0.0  &  1.6  &  0.1  \\
MPA1618-5147  &  1.8  &  0.1  &  2.2  &  0.4  &  1.6  &  0.0  &  1.2  &  0.1  &  1.5  &  0.2  \\
MPA1635-4458  &  2.3  &  0.1  &  2.1  &  0.4  &  1.9  &  0.4  &  1.6  &  0.0  &  1.6  &  0.0  \\
MPA1650-4747  &  3.1  &  0.5  &  3.3  &  0.4  &  3.3  &  0.2  &  3.4  &  0.1  &  3.5  &  0.2  \\
MPA1703-4450  &  2.3  &  0.0  &  2.4  &  0.1  &  2.2  &  0.0  &  2.1  &  0.0  &  2.3  &  0.2  \\
MPA1711-3112  &  -  &  -  &  -  &  -  &  2.9  &  0.4  &  2.4  &  0.5  &  2.2  &  0.5  \\
MPA1713-4015  &  -  &  -  &  -  &  -  &  2.7  &  0.0  &  2.4  &  0.0  &  2.2  &  0.0  \\
MPA1717-3945  &  -  &  -  &  -  &  -  &  2.5  &  0.0  &  2.5  &  0.0  &  2.7  &  0.8  \\
MPA1719-3247  &  -  &  -  &  4.7  &  0.2  &  -  &  -  &  -  &  -  &  -  &  -  \\
MPA1725-3033  &  1.7  &  0.4  &  1.7  &  0.3  &  2.4  &  0.1  &  2.0  &  0.1  &  1.7  &  0.4  \\
MPA1728-3132  &  -  &  -  &  -  &  -  &  2.2  &  0.0  &  2.1  &  0.0  &  2.2  &  0.0  \\
MPA1729-3016  &  2.0  &  0.3  &  1.8  &  0.3  &  1.5  &  0.0  &  1.5  &  0.0  &  1.3  &  0.1  \\
MPA1736-3717  &  -  &  -  &  -  &  -  &  1.2  &  0.1  &  -  &  -  &  1.5  &  n  \\
MPA1737-3837  &  -  &  -  &  -  &  -  &  3.7  &  0.7  &  2.9  &  0.5  &  2.6  &  0.8  \\
MPA1739-2648  &  1.9  &  0.0  &  1.8  &  0.1  &  1.3  &  0.1  &  1.1  &  0.0  &  1.1  &  0.0  \\
MPA1742-2613  &  2.0  &  0.3  &  1.7  &  0.2  &  1.2  &  0.0  &  1.2  &  0.1  &  1.1  &  0.1  \\
MPA1744-3444  &  1.8  &  0.1  &  2.0  &  n  &  2.3  &  0.1  &  2.0  &  0.2  &  2.2  &  0.3  \\
MPA1747-2649  &  -  &  -  &  -  &  -  &  1.6  &  0.0  &  1.5  &  0.0  &  1.6  &  0.1  \\
MPA1751-2223  &  -  &  -  &  -  &  -  &  1.5  &  0.1  &  1.7  &  0.3  &  1.6  &  0.2  \\
MPA1751-2838  &  -  &  -  &  -  &  -  &  1.8  &  0.0  &  1.6  &  0.1  &  1.7  &  0.1  \\
MPA1751-3339  &  1.4  &  0.1  &  1.3  &  0.1  &  1.2  &  0.1  &  1.2  &  0.1  &  1.3  &  0.1  \\
MPA1755-2212  &  2.4  &  0.6  &  2.1  &  0.7  &  1.6  &  0.0  &  1.5  &  0.0  &  1.5  &  0.1  \\
MPA1755-2741  &  -  &  -  &  -  &  -  &  1.2  &  0.0  &  1.4  &  0.1  &  1.3  &  0.1  \\
MPA1757-3410  &  -  &  -  &  -  &  -  &  1.4  &  0.2  &  1.4  &  0.2  &  1.1  &  0.2  \\
MPA1800-3023  &  -  &  -  &  1.1  &  0.1  &  -  &  -  &  -  &  -  &  -  &  -  \\
MPA1815-2113  &  3.0  &  0.1  &  2.8  &  0.1  &  2.9  &  0.0  &  2.5  &  0.0  &  2.9  &  0.1  \\
NGC 6644  &  3.5  &  0.1  &  3.3  &  0.0  &  2.6  &  0.1  &  2.2  &  0.0  &  2.3  &  0.2  \\
Pe 1-7  &  2.2  &  0.0  &  2.1  &  0.1  &  2.0  &  0.0  &  2.3  &  0.0  &  2.2  &  0.2  \\
Pe 1-9  &  1.6  &  0.1  &  1.4  &  0.1  &  1.2  &  0.0  &  1.1  &  0.0  &  1.1  &  0.1  \\
Pe 2-8  &  2.1  &  0.0  &  2.1  &  0.0  &  2.2  &  0.2  &  2.2  &  0.3  &  2.3  &  0.3  \\
Pe 2-10  &  -  &  -  &  -  &  -  &  1.2  &  0.0  &  1.3  &  0.1  &  1.3  &  0.1  \\
PHR1202-6112  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  1.2  &  0.2  \\
PHR1213-6344  &  1.5  &  0.1  &  1.4  &  0.1  &  1.6  &  0.4  &  1.4  &  0.2  &  1.4  &  0.1  \\
PHR1223-6236  &  1.5  &  n  &  1.5  &  0.1  &  1.3  &  0.1  &  1.2  &  0.1  &  1.3  &  0.1  \\
PHR1250-6346  &  1.1  &  n  &  0.9  &  n  &  1.2  &  0.2  &  1.2  &  0.0  &  1.1  &  0.1  \\
PHR1257-6052  &  0.9  &  n  &  1.2  &  0.2  &  1.2  &  0.2  &  1.1  &  0.1  &  1.3  &  0.2  \\
PHR1318-6358  &  1.3  &  0.1  &  1.6  &  0.3  &  1.5  &  0.3  &  1.3  &  0.1  &  1.2  &  0.1  \\
PHR1324-6418  &  1.7  &  0.2  &  1.6  &  0.2  &  1.1  &  0.1  &  1.1  &  0.1  &  1.2  &  0.1  \\
PHR1324-6448  &  2.0  &  0.4  &  1.9  &  0.4  &  1.5  &  0.1  &  1.4  &  0.1  &  1.3  &  0.1  \\
PHR1327-6032  &  1.8  &  0.2  &  1.9  &  0.3  &  1.8  &  0.1  &  2.1  &  0.2  &  1.4  &  0.4  \\
PHR1335-6015  &  2.1  &  0.0  &  1.7  &  0.0  &  1.6  &  n  &  1.8  &  0.1  &  1.5  &  0.3  \\
PHR1341-6427  &  -  &  -  &  -  &  -  &  -  &  -  &  1.1  &  0.0  &  2.0  &  0.3  \\
PHR1408-6229  &  2.4  &  0.6  &  2.1  &  0.4  &  2.5  &  0.5  &  2.6  &  0.6  &  1.8  &  0.8  \\
PHR1420-5933  &  2.6  &  0.2  &  3.3  &  0.3  &  1.1  &  0.1  &  2.1  &  0.6  &  2.4  &  0.8  \\
PHR1438-6140  &  1.7  &  n  &  1.1  &  n  &  1.4  &  0.0  &  1.0  &  n  &  1.3  &  0.1  \\
PHR1447-6127  &  -  &  -  &  -  &  -  &  1.3  &  n  &  1.3  &  0.0  &  1.1  &  0.1  \\
PHR1453-5714  &  2.1  &  0.7  &  2.1  &  0.7  &  1.2  &  0.0  &  1.2  &  0.1  &  1.2  &  0.2  \\
PHR1507-5925  &  2.1  &  0.1  &  2.1  &  0.1  &  2.0  &  0.1  &  1.9  &  0.4  &  2.0  &  0.2  \\
PHR1539-5727  &  2.3  &  0.7  &  2.0  &  0.5  &  1.4  &  0.1  &  1.4  &  0.0  &  1.4  &  0.1  \\
PHR1551-5653  &  1.7  &  0.0  &  1.5  &  0.0  &  1.4  &  0.1  &  1.2  &  0.0  &  1.2  &  0.1  \\
PHR1552-5254  &  1.0  &  n  &  1.4  &  0.3  &  1.3  &  0.3  &  1.2  &  0.2  &  1.3  &  0.3  \\
PHR1557-5128  &  1.6  &  0.3  &  1.6  &  0.1  &  1.6  &  0.1  &  1.8  &  0.5  &  1.4  &  0.2  \\
PHR1619-4907  &  -  &  -  &  -  &  -  &  -  &  -  &  1.1  &  n  &  0.9  &  0.0  \\
PHR1633-4650  &  -  &  -  &  1.5  &  0.1  &  1.8  &  0.0  &  1.7  &  0.1  &  1.6  &  0.2  \\
PHR1634-4628  &  1.4  &  0.1  &  1.4  &  0.0  &  1.3  &  0.0  &  1.3  &  0.0  &  1.2  &  0.0  \\
PHR1639-4516  &  -  &  -  &  1.5  &  n  &  1.0  &  0.1  &  1.0  &  0.1  &  1.0  &  0.1  \\
PHR1704-3819  &  1.9  &  0.1  &  1.7  &  0.1  &  1.5  &  0.3  &  1.4  &  0.2  &  1.5  &  0.2  \\
PHR1707-4309  &  2.1  &  0.3  &  1.9  &  0.3  &  1.6  &  0.0  &  1.4  &  0.1  &  1.7  &  0.3  \\
PHR1709-3931  &  1.3  &  0.0  &  1.3  &  0.0  &  1.3  &  0.1  &  1.3  &  0.2  &  1.3  &  0.2  \\
PHR1712-3452  &  1.6  &  0.0  &  1.7  &  0.0  &  1.7  &  0.1  &  1.5  &  0.1  &  1.6  &  0.1  \\
PHR1714-4006  &  -  &  -  &  -  &  -  &  2.3  &  0.3  &  2.3  &  0.4  &  2.5  &  0.3  \\
PHR1735-2527  &  -  &  -  &  -  &  -  &  1.0  &  n  &  -  &  -  &  1.1  &  n  \\
PHR1752-3244  &  1.1  &  0.1  &  1.1  &  0.1  &  1.0  &  0.1  &  1.0  &  0.1  &  0.9  &  0.0  \\
PHR1801-2522  &  -  &  -  &  -  &  -  &  4.2  &  0.4  &  4.6  &  0.3  &  4.1  &  0.4  \\
PHR1802-2637  &  1.8  &  0.0  &  1.8  &  0.0  &  1.1  &  0.1  &  1.0  &  0.1  &  1.0  &  0.1  \\
PHR1804-2653  &  1.5  &  0.4  &  1.9  &  0.2  &  1.9  &  0.1  &  1.9  &  0.1  &  1.2  &  0.2  \\
PHR1804-2913  &  2.3  &  0.0  &  2.0  &  0.1  &  1.7  &  0.5  &  1.6  &  0.4  &  1.4  &  0.3  \\
PN 1231-6401  &  2.2  &  0.2  &  2.6  &  0.0  &  2.4  &  0.0  &  2.2  &  0.0  &  1.9  &  0.1  \\
PN 1412-5947  &  2.8  &  0.2  &  2.7  &  0.2  &  2.3  &  0.1  &  2.1  &  0.1  &  2.0  &  0.2  \\
PN 1434-5858  &  2.7  &  0.2  &  2.3  &  0.0  &  1.8  &  0.1  &  1.7  &  0.1  &  1.8  &  0.2  \\
PN 1557-5445  &  2.1  &  0.0  &  2.1  &  0.1  &  1.7  &  0.0  &  1.5  &  0.0  &  1.5  &  0.1  \\
PN 1600-5041  &  1.7  &  0.2  &  1.5  &  0.1  &  1.4  &  0.2  &  1.2  &  0.1  &  1.3  &  0.1  \\
PN 1652-4341  &  4.1  &  0.0  &  3.5  &  0.6  &  3.7  &  0.0  &  3.7  &  0.0  &  3.8  &  0.3  \\
PN 1708-4227  &  2.3  &  0.1  &  2.2  &  0.1  &  1.8  &  0.1  &  1.6  &  0.1  &  1.6  &  0.0  \\
PPA1704-3824  &  3.7  &  0.3  &  3.2  &  0.9  &  3.2  &  0.9  &  3.3  &  0.9  &  4.1  &  0.8  \\
PPA1705-3748  &  2.8  &  0.0  &  3.1  &  0.0  &  3.0  &  0.2  &  2.6  &  0.3  &  2.8  &  0.4  \\
PPA1715-3313  &  -  &  -  &  2.4  &  0.3  &  -  &  -  &  -  &  -  &  -  &  -  \\
PPA1718-3315  &  1.8  &  0.2  &  1.8  &  0.1  &  -  &  -  &  -  &  -  &  -  &  -  \\
PPA1721-3149  &  3.2  &  0.0  &  3.4  &  0.1  &  -  &  -  &  -  &  -  &  -  &  -  \\
PPA1722-3139  &  2.9  &  0.0  &  2.8  &  0.1  &  -  &  -  &  -  &  -  &  -  &  -  \\
PPA1722-3317  &  3.1  &  0.3  &  2.8  &  0.1  &  2.9  &  0.0  &  1.5  &  0.1  &  2.1  &  0.8  \\
PPA1723-3038  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  2.5  &  n  \\
PPA1724-3043  &  2.5  &  0.4  &  2.4  &  0.3  &  1.8  &  0.0  &  1.7  &  0.1  &  1.6  &  0.1  \\
PPA1725-3216  &  2.0  &  0.2  &  2.6  &  0.8  &  -  &  -  &  -  &  -  &  -  &  -  \\
PPA1726-3045  &  3.2  &  0.7  &  3.4  &  0.5  &  3.5  &  0.0  &  3.4  &  0.3  &  3.0  &  0.4  \\
PPA1729-2611  &  -  &  -  &  -  &  -  &  3.8  &  0.0  &  3.6  &  0.1  &  3.7  &  0.1  \\
PPA1730-2621  &  -  &  -  &  -  &  -  &  1.5  &  0.0  &  1.3  &  0.0  &  1.7  &  0.2  \\
PPA1734-3004  &  -  &  -  &  -  &  -  &  1.5  &  0.0  &  1.4  &  0.0  &  1.7  &  0.3  \\
PPA1734-3102  &  -  &  -  &  -  &  -  &  2.5  &  0.2  &  2.7  &  0.2  &  2.7  &  0.1  \\
PPA1735-2809  &  3.2  &  0.1  &  2.6  &  0.2  &  -  &  -  &  -  &  -  &  -  &  -  \\
PPA1737-3414  &  -  &  -  &  -  &  -  &  1.6  &  0.3  &  1.3  &  0.2  &  2.0  &  0.2  \\
PPA1737-3650  &  -  &  -  &  -  &  -  &  1.6  &  0.0  &  1.5  &  0.0  &  1.7  &  0.0  \\
PPA1738-3753  &  -  &  -  &  -  &  -  &  1.8  &  0.0  &  1.8  &  0.0  &  1.8  &  0.0  \\
PPA1740-2708  &  1.2  &  0.1  &  -  &  -  &  1.2  &  0.1  &  -  &  -  &  1.3  &  0.3  \\
PPA1741-2332  &  1.0  &  0.1  &  1.0  &  0.1  &  0.9  &  0.1  &  0.9  &  0.1  &  1.0  &  0.1  \\
PPA1741-3405  &  1.2  &  n  &  1.8  &  0.5  &  3.1  &  0.4  &  1.6  &  0.1  &  1.6  &  0.4  \\
PPA1743-3315  &  3.7  &  0.8  &  3.7  &  0.8  &  3.3  &  0.4  &  1.4  &  0.2  &  2.8  &  0.2  \\
PPA1746-3454  &  1.6  &  0.0  &  1.5  &  0.0  &  1.5  &  0.1  &  1.2  &  0.1  &  1.2  &  0.0  \\
PPA1747-3215  &  2.0  &  0.2  &  2.4  &  0.0  &  2.5  &  0.0  &  2.2  &  0.0  &  2.0  &  0.6  \\
PPA1750-3152  &  -  &  -  &  1.1  &  n  &  -  &  -  &  -  &  -  &  -  &  -  \\
PPA1756-2311  &  1.9  &  n  &  -  &  -  &  1.4  &  0.0  &  1.6  &  0.3  &  -  &  -  \\
PPA1800-2904  &  1.1  &  n  &  1.1  &  n  &  -  &  -  &  -  &  -  &  1.5  &  n  \\
PPA1801-2553  &  2.7  &  0.0  &  2.6  &  0.0  &  2.8  &  0.7  &  2.7  &  0.1  &  2.7  &  0.1  \\
PPA1803-2516  &  2.1  &  0.1  &  1.8  &  0.1  &  1.2  &  0.0  &  1.6  &  0.1  &  1.3  &  0.1  \\
PPA1803-2826  &  2.8  &  0.2  &  2.1  &  0.3  &  2.3  &  0.3  &  1.6  &  0.1  &  1.4  &  0.2  \\
PPA1809-3233  &  -  &  -  &  -  &  -  &  1.6  &  0.3  &  1.3  &  0.1  &  1.1  &  0.1  \\
PPA1813-2233  &  2.1  &  0.7  &  2.9  &  0.1  &  2.2  &  0.7  &  1.7  &  0.7  &  1.6  &  0.7  \\
PPA1831-2356  &  -  &  -  &  -  &  -  &  1.3  &  0.5  &  1.6  &  0.2  &  1.4  &  0.3  \\
Sa 2-215  &  -  &  -  &  -  &  -  &  1.9  &  0.1  &  2.1  &  0.1  &  1.9  &  0.1  \\
Sa 3-92  &  2.7  &  0.8  &  2.3  &  0.9  &  -  &  -  &  2.1  &  n  &  1.9  &  0.4  \\
Sa 3-104  &  1.7  &  0.0  &  1.6  &  0.1  &  1.9  &  0.3  &  1.6  &  0.1  &  1.6  &  0.0  \\
SAWI 5  &  -  &  -  &  -  &  -  &  1.4  &  0.1  &  1.2  &  0.1  &  1.4  &  0.1  \\
SAWI 7  &  -  &  -  &  -  &  -  &  1.5  &  0.2  &  1.4  &  0.1  &  1.5  &  0.1  \\
SB 1  &  2.5  &  0.2  &  2.5  &  0.0  &  2.2  &  0.2  &  -  &  -  &  -  &  -  \\
SB 4  &  1.4  &  0.1  &  1.3  &  0.1  &  1.3  &  0.1  &  1.1  &  0.1  &  1.0  &  0.1  \\
SB 5  &  -  &  -  &  -  &  -  &  1.2  &  0.1  &  1.1  &  0.0  &  1.1  &  0.0  \\
SB 9  &  -  &  -  &  1.0  &  n  &  1.2  &  n  &  1.0  &  n  &  -  &  -  \\
SB 12  &  -  &  -  &  -  &  -  &  1.7  &  0.0  &  1.8  &  0.0  &  1.5  &  0.1  \\
SB 14  &  -  &  -  &  -  &  -  &  1.3  &  0.1  &  1.1  &  0.2  &  1.0  &  0.1  \\
SB 16  &  2.5  &  0.0  &  2.5  &  0.0  &  2.5  &  0.0  &  2.1  &  0.2  &  1.5  &  0.2  \\
SB 37  &  -  &  -  &  -  &  -  &  3.7  &  0.7  &  3.6  &  0.6  &  3.3  &  0.4  \\
SB 38  &  1.9  &  0.1  &  1.8  &  0.1  &  1.7  &  0.1  &  1.6  &  0.1  &  1.3  &  0.1  \\
SB 39  &  2.2  &  0.3  &  2.1  &  0.5  &  1.4  &  0.1  &  1.1  &  0.1  &  1.2  &  0.2  \\
SB 49  &  3.0  &  0.1  &  2.9  &  0.1  &  1.7  &  0.0  &  1.5  &  0.1  &  1.5  &  0.1  \\
SB 51  &  -  &  -  &  -  &  -  &  1.6  &  0.4  &  1.3  &  0.2  &  1.4  &  0.2  \\
SB 54  &  -  &  -  &  -  &  -  &  1.6  &  0.2  &  1.3  &  0.2  &  1.3  &  0.2  \\
SB 55  &  1.6  &  0.0  &  1.7  &  0.1  &  1.3  &  0.1  &  1.1  &  0.0  &  1.1  &  0.1  \\
SB 56  &  -  &  -  &  -  &  -  &  2.2  &  0.7  &  1.9  &  0.4  &  1.7  &  0.3  \\
SrWe 2  &  -  &  -  &  -  &  -  &  1.5  &  0.0  &  1.4  &  0.1  &  1.4  &  0.1  \\
SwSt 1  &  3.9  &  0.9  &  3.1  &  0.9  &  2.7  &  0.5  &  2.2  &  0.2  &  2.5  &  0.2  \\
Ta 137  &  1.9  &  n  &  1.0  &  n  &  -  &  -  &  -  &  -  &  -  &  -  \\
Ta 140  &  -  &  -  &  -  &  -  &  1.4  &  0.0  &  1.5  &  0.1  &  1.7  &  0.2  \\
Ta 1567  &  -  &  -  &  -  &  -  &  0.9  &  n  &  1.0  &  0.1  &  -  &  -  \\
Ta 2337  &  -  &  -  &  -  &  -  &  1.3  &  0.1  &  1.1  &  0.0  &  1.1  &  0.0  \\
Th 3-4  &  2.0  &  0.0  &  2.6  &  0.6  &  -  &  -  &  -  &  -  &  -  &  -  \\
Th 3-6  &  3.1  &  0.0  &  3.2  &  0.1  &  -  &  -  &  -  &  -  &  -  &  -  \\
Th 3-10  &  3.4  &  0.1  &  3.6  &  0.4  &  3.7  &  0.0  &  3.7  &  0.0  &  3.1  &  0.6  \\
Th 3-11  &  2.5  &  n  &  2.9  &  0.7  &  -  &  -  &  -  &  -  &  -  &  -  \\
Th 3-12  &  2.4  &  0.2  &  2.3  &  0.3  &  2.5  &  0.1  &  2.1  &  0.1  &  1.7  &  0.2  \\
Th 3-13  &  2.5  &  0.3  &  2.2  &  0.2  &  2.0  &  0.1  &  1.9  &  0.0  &  1.6  &  0.0  \\
Th 3-14  &  -  &  -  &  -  &  -  &  1.3  &  0.1  &  1.4  &  0.1  &  1.4  &  0.1  \\
Th 3-15  &  -  &  -  &  -  &  -  &  2.3  &  0.4  &  1.9  &  0.2  &  2.0  &  0.3  \\
Th 3-19  &  2.0  &  0.3  &  1.9  &  0.3  &  1.9  &  0.3  &  1.5  &  0.1  &  1.4  &  0.1  \\
Th 3-23  &  3.4  &  0.1  &  3.5  &  0.1  &  -  &  -  &  -  &  -  &  3.7  &  0.0  \\
Th 3-25  &  3.5  &  0.0  &  3.7  &  0.0  &  -  &  -  &  -  &  -  &  -  &  -  \\
Th 3-27  &  -  &  -  &  -  &  -  &  2.6  &  0.4  &  1.1  &  0.0  &  2.2  &  0.9  \\
Th 3-33  &  2.0  &  0.1  &  1.8  &  0.0  &  -  &  -  &  -  &  -  &  -  &  -  \\
Th 3-35  &  -  &  -  &  -  &  -  &  2.1  &  0.5  &  2.5  &  0.1  &  2.4  &  0.2  \\
Th 3-55  &  -  &  -  &  -  &  -  &  2.3  &  0.1  &  2.1  &  0.0  &  2.4  &  0.0  \\
Th 4-3  &  1.9  &  0.1  &  1.7  &  0.0  &  1.2  &  0.1  &  1.3  &  0.1  &  1.4  &  0.1  \\
Th 4-5  &  2.2  &  0.6  &  3.7  &  1.4  &  1.3  &  n  &  5.4  &  n  &  -  &  -  \\
Th 4-6  &  2.5  &  0.5  &  2.5  &  0.7  &  1.9  &  0.1  &  1.6  &  0.0  &  1.6  &  0.0  \\
Th 4-9  &  1.6  &  0.0  &  1.6  &  0.0  &  1.3  &  0.1  &  1.2  &  0.1  &  1.3  &  0.2  \\
VB 2  &  2.7  &  0.7  &  2.2  &  0.4  &  1.6  &  0.1  &  1.4  &  0.1  &  1.4  &  0.1  \\
VB 3  &  2.0  &  0.2  &  -  &  -  &  1.8  &  0.2  &  1.4  &  0.2  &  1.4  &  0.3  \\
VBRC 7  &  -  &  -  &  -  &  -  &  -  &  -  &  1.0  &  n  &  -  &  -  \\
Vd 1-8  &  2.4  &  0.1  &  2.3  &  0.0  &  2.2  &  0.1  &  2.1  &  0.1  &  2.0  &  0.1  \\
Vd 1-9  &  2.5  &  0.3  &  2.4  &  0.2  &  2.1  &  0.0  &  2.0  &  0.0  &  2.1  &  0.1  \\
Vy 2-1  &  -  &  -  &  -  &  -  &  3.2  &  0.0  &  3.1  &  0.1  &  3.0  &  0.0  \\
WeKG 2  &  1.3  &  0.1  &  1.3  &  0.1  &  1.1  &  0.0  &  1.1  &  0.0  &  1.3  &  0.2  \\
WeKG 3  &  1.3  &  0.1  &  1.2  &  0.1  &  1.1  &  0.0  &  1.1  &  0.0  &  1.4  &  0.2  \\
\end{longtable}
\end{landscape}
}% End \longtabL






==> cds/table-5.tex <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\longtabL{5}{
\begin{landscape}
\begin{longtable}{lcccc}
\caption{\label{tablita-2} Planetary nebulae that were not measured.}\\
\hline\hline
name & PN G & $\alpha$(2000) & $\delta$(2000) & status  \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
name & PN G & $\alpha$(2000) & $\delta$(2000) & status  \\
\hline
\endhead
\hline
\endfoot
%%
JaSt 93        & 000.1$-$01.9  & 17 53 24.43  & $-$29 49 47.7 & N/D \\
Bl 3-10        & 000.1$-$02.3 & 17 55 20.48  & $-$29 57 33.4  & N/D \\
K 6-8          & 000.2+01.7  & 17 39 39.253  & $-$27 47 23.56  & N/D \\
PHR1752-2930 & 000.3$-$01.6 & 17 52 52.20  & $-$29 30 00.1  & N/D \\
JaSt 86        & 000.3$-$01.6  & 17 52 52.20  & $-$29 30 00.1 & N/D \\
Sa 3-117       & 000.3$-$02.8 & 17 57 43.367  & $-$30 02 29.91  & N/D \\
M 3-47         & 000.3$-$04.6 & 18 05 02.695  & $-$30 58 17.39  & ext \\
M 2-20         & 000.4$-$02.9 & 17 58 19.337  & $-$30 00 39.32  & N/D \\
JaSt 96  & 000.5$-$01.7  & 17 25 03.470  & $-$31 28 38.50 & N/D \\
Ae 2-Q         & 000.5$-$03.1 & 17 59 15.585  & $-$30 02 47.15 & N/D \\
SB 2           & 000.5$-$05.3  & 18 08 34.7  & $-$31 06 52  & N/D \\
JaSt 77        & 000.6$-$01.0  & 17 51 11.504  & $-$28 56 26.16 & N/D \\
KnFs 1         & 000.6$-$01.3 & 17 52 35.87  & $-$29 06 38.6 & N/D \\
SB 3           & 000.7$-$06.1  & 18 12 14.48  & $-$31 19 58.0  & N/D \\
M 2-35         & 000.7$-$07.4 & 18 17 37.195  & $-$31 56 46.86  & ext \\
JaSt 38 & 000.8+01.3  & 17 42 32.674  & $-$27 33 08.82  & N/D \\
JaSt 44 & 000.9+01.1  & 17 43 23.305  & $-$27 34 03.57 & N/D \\
PHR1804-3016 & 000.9$-$04.2 & 18 04 48.1  & $-$30 16 49  & N/D \\
M 3-23         & 000.9$-$04.8 & 18 07 06.148  & $-$30 34 16.96  & ext \\
JaSt 41        & 001.0+01.3  & 17 42 49.96  & $-$27 21 19.7 & N/D \\
K 1-4          & 001.0+01.9 & 17 40 27.366  & $-$27 01 02.91  & N/D \\
JaSt 89 & 001.3$-$01.0  & 17 53 06.57  & $-$28 18 09.2 & N/D \\
SAWI 1         & 001.4$-$03.4 & 18 02 25.85  & $-$29 25 05.4 & N/D \\
K 6-17         & 001.5$-$00.7  & 17 52 08.717  & $-$28 02 16.56  & N/D \\
JaSt 55        & 001.6+00.9  & 17 45 37.36  & $-$27 01 18.4 & N/D \\
K 6-10         & 001.6+01.5  & 17 43 16.950  & $-$26 44 17.54  & N/D \\
Bl Q           & 001.6$-$01.3 & 17 54 34.94  & $-$28 12 43.3  & N/D \\
SB 6           & 001.6$-$05.9  & 18 13 15.842  & $-$30 25 58.49  & N/D \\
H 1-45         & 002.0$-$02.0 & 17 58 21.87  & $-$28 14 52.3  & ext \\
KnFs 2         & 002.2$-$02.5 & 18 00 59.92  & $-$28 16 19.8  & N/D \\
PHR1808-2913 & 002.2$-$04.3 & 18 08 06.42  & $-$29 13 15.7 & N/D \\
Cn 1-5         & 002.2$-$09.4 & 18 29 11.675  & $-$31 29 58.81  & ext \\
PHR1744-2603 & 002.3+01.7 & 17 44 35.4  & $-$26 03 36  & N/D \\
Ta 5           & 002.3+02.2 & 17 42 30.10  & $-$25 45 28.7  & N/D \\
PPA1741-2538 & 002.3+02.4 & 17 41 48.4  & $-$25 38 18  & N/D \\
Sa 3-115       & 002.4$-$03.2 & 18 04 05.438  & $-$28 27 50.90  & N/D \\
Pe 2-11        & 002.5$-$01.7 & 17 58 31.27  & $-$27 37 05.8  & S/D \\
Ta 1580        & 002.6+02.1 & 17 43 39.442  & $-$25 36 42.51  & N/D \\
PPA1745-2542 & 002.7+01.7 & 17 45 18.9  & $-$25 42 05  & N/D \\
M 1-42         & 002.7$-$04.8 & 18 11 05.07  & $-$28 58 58.5  & ext \\
Pe 2-12        & 002.8$-$02.2 & 18 01 10.300  & $-$27 38 19.88  & S/D \\
Hb 4           & 003.1+02.9 & 17 41 52.763  & $-$24 42 08.07 & ext \\
K 5-7          & 003.1+04.1  & 17 37 20.167  & $-$24 03 27.84  & N/D \\
SB 7           & 003.3$-$06.1  & 18 17 46.363  & $-$29 06 07.52 & N/D \\
MPA1748-2511 & 003.5+01.3 & 17 48 41.629  & $-$25 11 33.37  & ext \\
NGC 6565       & 003.5$-$04.6 & 18 11 52.470  & $-$28 10 42.27 & ext \\
PHR1759-2630 & 003.6$-$01.3 & 17 59 12.09  & $-$26 30 24.8  & ext \\
Ta 2111        & 003.9+01.6 & 17 48 28.465  & $-$24 41 25.07  & N/D \\
M 1-35         & 003.9$-$02.3 & 18 03 39.30  & $-$26 43 33.9 & ext \\
KnFs 7         & 003.9$-$03.1 & 18 06 50.05  & $-$27 06 16.09  & S/D \\
M 2-29         & 004.0$-$03.0 & 18 06 40.862  & $-$26 54 55.95  & S/D \\
Pe 1-12        & 004.0$-$05.8 & 18 17 42.37  & $-$28 17 16.5  & N/D \\
KnFs 10        & 004.2$-$03.2 & 18 08 01.312  & $-$26 54 01.52 & S/D \\
SB 8           & 004.2$-$05.2  & 18 15 50.3  & $-$27 49 00  & N/D \\
H 1-53         & 004.3$-$02.6 & 18 05 57.43  & $-$26 29 42.0 & S/D \\
MPA1748-2402 & 004.5+02.0 & 17 48 21.26  & $-$24 02 14.0  & N/D \\
SB 10          & 004.7$-$05.5  & 18 18 06.9  & $-$27 31 35  & N/D \\
M 1-25         & 004.9+04.9 & 17 38 30.32  & $-$22 08 38.8 & ext \\
H 1-27         & 005.0+04.4 & 17 40 17.95  & $-$22 19 18.0  & S/D \\
M 3-13         & 005.2+04.2 & 17 41 36.62  & $-$22 13 03.0 & S/D \\
SB 11          & 005.2$-$05.9  & 18 20 44.7  & $-$27 15 48  & N/D \\
M 3-24         & 005.5$-$02.5 & 18 07 53.914  & $-$25 24 02.71  & ext \\
H 2-44         & 005.5$-$04.0 & 18 13 40.45  & $-$26 08 38.3 & N/D \\
NGC 6620       & 005.8$-$06.1 & 18 22 54.17  & $-$26 49 17.1  & ext \\
KnFs 15        & 006.2$-$03.7 & 18 14 19.324  & $-$25 20 51.22  & N/D \\
H 2-18         & 006.3+04.4 & 17 43 28.751  & $-$21 09 51.29  & S/D \\
Pe 2-13        & 006.4$-$04.6 & 18 18 13.41  & $-$25 38 10.4 & N/D \\
M 1-41         & 006.7$-$02.2 & 18 09 29.902  & $-$24 12 23.46  & N/D \\
Th 4-7         & 006.8+02.3 & 17 52 22.569  & $-$21 51 13.43  & ext \\
M 3-15         & 006.8+04.1 & 17 45 31.74  & $-$20 58 01.8 & ext \\
Hb 6           & 007.2+01.8 & 17 55 07.023  & $-$21 44 39.98  & ext \\
Th 4-1         & 007.5+04.3 & 17 46 20.82  & $-$20 13 48.3 & S/D \\
H 1-65         & 007.8$-$04.4 & 18 20 08.85  & $-$24 15 05.0 & S/D \\
NGC 6445       & 008.0+03.9 & 17 49 15.21  & $-$20 00 34.5  & ext \\
M 1-40         & 008.3$-$01.1 & 18 08 25.994  & $-$22 16 53.25  & ext \\
He 2-406       & 008.6$-$07.0 & 18 31 52.845  & $-$24 46 16.55  & ext \\
PHR1751-1925 & 008.8+03.8 & 17 51 08.7  & $-$19 25 47  & N/D \\
NGC 6629       & 009.4$-$05.0 & 18 25 42.458  & $-$23 12 10.23  & ext \\
M 3-32         & 009.4$-$09.8 & 18 44 43.03  & $-$25 21 34.8  & ext \\
H 1-67         & 009.8$-$04.6 & 18 25 04.976  & $-$22 34 52.64  & ext \\
IRAS18333-2357 & 009.8$-$07.5 & 18 36 22.85  & $-$23 55 19.5  & N/D \\
BMP1145-6328 & 295.6$-$01.5 & 11 45 09.4 & $-$63 28 54 & N/D \\
PHR1206-6122 & 297.5+01.0 & 12 06 25.5 & $-$61 22 44 & N/D \\
PHR1203-6403 & 297.6$-$01.6 & 12 03 12.4 & $-$64 03 41 & N/D \\
PHR1212-6043 & 298.2+01.8 & 12 12 48.4 & $-$60 43 15 & N/D \\
He 2-76        & 298.2$-$01.7  & 12 08.4 & $-$64 12 & ext \\
PHR1216-6039 & 298.6+01.9 & 12 16 09.1 & $-$60 39 32 & N/D \\
PHR1212-6407 & 298.6$-$01.5 & 12 12 28.0 & $-$64 07 11 & N/D \\
He 2-81        & 299.8$-$01.3  & 12 23.0 & $-$64 02 & ext \\
He 2-83        & 300.2+00.6  & 12 28.7 & $-$62 06 & ext \\
He 2-85        & 300.5$-$01.1  & 12 30.1 & $-$63 53 & ext \\
He 2-86        & 300.7$-$02.0  & 12 30.5 & $-$64 53 & ext \\
MPA1239-6048 & 301.5+02.0 & 12 39 46.3 & $-$60 48 17 & ext \\
PHR1244-6231 & 302.1+00.3 & 12 44 28.5 & $-$62 31 19 & N/D \\
PHR1246-6324 & 302.3$-$00.5 & 12 46 26.5 & $-$63 24 28 & ext \\
VBRC 4         & 302.6$-$00.9  & 12 48.5 & $-$63 50 & N/D \\
PHR1309-6457 & 304.7$-$02.1 & 13 09 01.7 & $-$64 57 18 & N/D \\
MPA1315-6338 & 305.6$-$00.9 & 13 15 30.4 & $-$63 38 43 & ext \\
Th 2-A         & 306.4$-$00.6  & 13 22.5 & $-$63 21 & N/D \\
BMP1322-6330 & 306.4$-$00.8 & 13 22 55.4 & $-$63 30 34 & N/D \\
MPA1324-6320 & 306.6$-$00.7 & 13 24 16.8 & $-$63 20 06 & N/D \\
MPA1330-6438 & 307.0$-$02.0 & 13 30 11.0 & $-$64 38 27 & N/D \\
PHR1326-6103 & 307.1+01.5 & 13 26 21.7 & $-$61 03 08 & N/D \\
PHR1332-6412 & 307.3$-$01.6 & 13 32 05.7 & $-$64 12 30 & N/D \\
MPA1337-6258 & 308.1$-$00.5 & 13 37 54.9 & $-$62 58 54 & ext \\
VBRC 5         & 309.2+01.3  & 13 44.0 & $-$60 50 & N/D \\
Vo 4           & 310.4+01.3  & 13 53.4 & $-$60 34 & ext \\
PHR1408-6106 & 312.1+00.3 & 14 08 51.7 & $-$61 06 27 & N/D \\
He 2-107       & 312.6$-$01.8  & 14 18.7 & $-$63 07 & ext \\
BMP1423-5923 & 314.4+01.3 & 14 23 59.7 & $-$59 23 38 & ext \\
PN 1417-5824   & 314.4+02.2  & 14 21.3 & $-$58 39 & ext \\
PHR1432-6138 & 314.5$-$01.0 & 14 32 05.0 & $-$61 38 42 & N/D \\
He 2-111       & 315.0$-$00.3  & 14 33.3 & $-$60 50 & ext \\
LoTr 9         & 315.7$-$01.2  & 14 41.3 & $-$61 20 & N/D \\
PHR1437-5949 & 315.9+00.3 & 14 37 53.2 & $-$59 49 25 & N/D \\
LoTr 10        & 316.3$-$01.3  & 14 46.3 & $-$61 14 & N/D \\
MPA1440-5802 & 316.9+01.8 & 14 40 27.4 & $-$58 02 19 & ext \\
He 2-114       & 318.3$-$02.0  & 15 04.2 & $-$60 54 & ext \\
PHR1457-5812 & 318.9+00.7 & 14 57 35.7 & $-$58 12 09 & ext \\
He 2-120       & 321.8+01.9  & 15 12.0 & $-$55 40 & ext \\
BMP1525-5823 & 322.0$-$01.3 & 15 25 59.4 & $-$58 23 02 & ext \\
MPA1525-5528 & 323.5+01.1 & 15 25 06.1 & $-$55 28 22 & N/D \\
MPA1539-5709 & 324.1$-$01.3 & 15 39 10.6 & $-$57 09 51 & N/D \\
PHR1548-5629 & 325.5$-$01.6 & 15 48 21.3 & $-$56 29 56 & N/D \\
FP1550-5639 & 325.6$-$01.8 & 15 50 04.6 & $-$56 39 13 & N/D \\
BMP1533-5319 & 325.7+02.2 & 15 33 20.6 & $-$53 19 01 & ext \\
MPA1541-5243 & 327.1+01.9 & 15 41 29.5 & $-$52 43 49 & ext \\
MPA1559-5552 & 327.1$-$02.0 & 15 59 11.1 & $-$55 52 18 & N/D \\
PHR1547-5214 & 328.0+01.8 & 15 47 09.6 & $-$52 14 44 & N/D \\
Sp 1           & 329.0+01.9  & 15 51.6 & $-$51 31 & ext \\
HeFa 1         & 329.5$-$02.2  & 16 12.5 & $-$54 24 & S/D \\
BMP1613-5406 & 329.8$-$02.1 & 16 13 02.0 & $-$54 06 32 & N/D \\
PHR1616-5324 & 330.7$-$02.0 & 16 16 54.2 & $-$53 24 40 & N/D \\
PHR1603-5016 & 331.3+01.6 & 16 03 53.7 & $-$50 16 52 & ext \\
He 2-145       & 331.4+00.5  & 16 09.0 & $-$51 02 & ext \\
Mz 3           & 331.7$-$01.0  & 16 17.2 & $-$51 59 & ext \\
PHR1626-5216 & 332.5$-$02.2 & 16 26 24.2 & $-$52 16 58 & N/D \\
He 2-152       & 333.4+01.1  & 16 15.3 & $-$49 13 & ext \\
PHR1619-4914 & 333.9+00.6 & 16 19 40.1 & $-$49 14 00 & ext \\
MmWe 1-6       & 334.3$-$01.4  & 16 31.1 & $-$50 26 & ext \\
He 2-169       & 335.4$-$01.1  & 16 34.3 & $-$49 21 & ext \\
PHR1637-4957 & 335.4$-$01.9 & 16 37 44.9 & $-$49 57 50 & ext \\
Pe 1-6         & 336.2+01.9  & 16 23.9 & $-$46 42 & ext \\
BMP1636-4529 & 338.6+01.1 & 16 36 58.7 & $-$45 29 29 & N/D \\
MPA1657-4447 & 341.5$-$01.1 & 16 57 13.3 & $-$44 47 18 & N/D \\
PHR1702-4443 & 342.0$-$01.7 & 17 02 04.3 & $-$44 43 20 & N/D \\
H 1-3          & 342.7+00.7  & 16 53.5 & $-$42 39 & N/D \\
He 2-198       & 342.9$-$02.0  & 17 06.4 & $-$44 13 & ext \\
HtTr 5         & 343.3$-$00.6  & 17 01.5 & $-$43 06 & N/D \\
PHR1653-4143 & 343.5+01.2 & 16 53 55.3 & $-$41 44 00 & N/D \\
H 1-5          & 343.9+00.8  & 16 57.4 & $-$41 38 & ext \\
H 1-6          & 344.2$-$01.2  & 17 07.0 & $-$42 41 & ext \\
H 1-7          & 345.2$-$01.2  & 17 10.4 & $-$41 53 & ext \\
IC 4637        & 345.4+00.1  & 17 05.2 & $-$40 53 & ext \\
MPA1715-3903 & 348.0$-$00.3 & 17 15 16.1 & $-$39 03 48 & N/D \\
PHR1710-3732 & 348.7+01.3 & 17 10 12.3 & $-$37 32 51 & N/D \\
PHR1724-3859 & 349.1$-$01.7 & 17 24 30.7 & $-$38 59 44 & N/D \\
NGC 6337       & 349.3$-$01.1  & 17 22.2 & $-$38 29 & ext \\
NGC 6302       & 349.5+01.0  & 17 13.8 & $-$37 06 & ext \\
MPA1727-3851 & 349.6$-$02.1 & 17 27 36.8 & $-$38 51 09 & N/D \\
H 1-26         & 350.1$-$03.9 & 17 36 29.90  & $-$39 21 56.8  & ext \\
H 1-28         & 350.5$-$05.0 & 17 42 54.066  & $-$39 36 24.04  & ext \\
PPA1734-3817 & 350.8$-$03.0 & 17 34 52.8  & $-$38 17 19 & N/D \\
SB 33          & 351.2$-$06.3  & 17 50 27.700  & $-$39 40 17.40  & N/D \\
SB 34          & 351.5$-$06.5  & 17 52 09.386  & $-$39 32 14.52  & S/D \\
H 1-37         & 351.6$-$06.2 & 17 50 44.569  & $-$39 17 25.98  & ext \\
SB 35          & 351.7$-$06.6  & 17 53 02.87  & $-$39 24 08.9 & S/D \\
SB 36          & 352.0$-$06.7  & 17 54 20.83  & $-$39 10 37.9 & S/D \\
H 1-12         & 352.6+00.1 & 17 26 24.258  & $-$35 01 41.88 & ext \\
H 1-13         & 352.8$-$00.2 & 17 28 27.46  & $-$35 07 31.8  & ext \\
Fg 3           & 352.9$-$07.5 & 18 00 11.82  & $-$38 49 52.6 & S/D \\
H 1-38         & 353.2$-$05.2 & 17 50 45.216  & $-$37 23 54.18 & N/D \\
PPA1738-3546 & 353.3$-$02.2 & 17 38 16.2  & $-$35 46 27 & N/D \\
PPA1740-3551 & 353.5$-$02.6 & 17 40 21.4  & $-$35 51 31  & N/D \\
JaFu 2         & 353.5$-$05.0  & 17 50 11.1  & $-$37 03 27  & N/D \\
H 1-52         & 354.4$-$07.8 & 18 04 57.594  & $-$37 38 07.92  & S/D \\
PHR1722-3210 & 354.5+02.4 & 17 22 11.7  & $-$32 10 45  & N/D \\
PPA1740-3437 & 354.5$-$02.0a & 17 40 30.5  & $-$34 37 17  & N/D \\
Ta 139         & 354.6+04.9  & 17 12 53.539  & $-$30 40 05.70  & N/D \\
SB 40          & 354.7$-$07.2  & 18 02 55.69  & $-$37 08 13.1  & S/D \\
H 1-31         & 355.1$-$02.9 & 17 45 32.104  & $-$34 33 55.32  & N/D \\
M 3-21         & 355.1$-$06.9 & 18 02 32.33  & $-$36 39 11.3 & S/D \\
SB 42          & 355.3$-$07.5  & 18 05 52.556  & $-$36 45 37.40  & S/D \\
Ta 138         & 355.4+02.3  & 17 25 03.470  & $-$31 28 38.50  & ext \\
PHR1740-3324 & 355.6$-$01.4 & 17 40 54.9  & $-$33 24 18 & N/D \\
PHR1721-3027 & 355.8+03.5 & 17 21 31.7  & $-$30 27 20  & N/D \\
SB 43          & 355.8$-$08.7  & 18 12 23.684  & $-$36 52 53.72  & N/D \\
PPA1741-3302 & 356.0$-$01.4 & 17 41 33.4  & $-$33 02 15  & N/D \\
SB 44          & 356.0$-$07.4A & 18 07 07.953  & $-$36 02 45.64  & S/D \\
SB 45          & 356.0$-$07.4B & 18 06 52.495  & $-$36 06 42.82  & S/D \\
PPA1747-3341 & 356.1$-$02.7 & 17 47 04.8  & $-$33 41 03  & N/D \\
SB 46          & 356.1$-$08.6  & 18 12 39.873  & $-$36 31 49.16  & N/D \\
PPA1751-3401 & 356.2$-$03.6 & 17 51 06.9  & $-$34 01 41  & N/D \\
M 3-49         & 356.3$-$06.2 & 18 02 32.06  & $-$35 13 14.3  & S/D \\
SB 47          & 356.3$-$07.3  & 18 07 21.472  & $-$35 45 44.04  & N/D \\
SB 48          & 356.4$-$06.8  & 18 05 14.396  & $-$35 28 07.54  & S/D \\
H 1-57         & 356.6$-$07.8 & 18 09 49.240  & $-$35 44 13.32 & S/D \\
H 1-51         & 356.7$-$06.4 & 18 04 29.304  & $-$34 58 00.98 & S/D \\
M 4-4          & 357.0+02.4 & 17 28 50.29  & $-$30 07 45.1 & N/D \\
Th 3-24        & 357.1+01.9 & 17 30 51.354  & $-$30 17 12.49  & N/D \\
TaJu 18        & 357.1+04.4 & 17 21 37.90  & $-$28 55 13.9 & N/D \\
M 3-50         & 357.1$-$06.1 & 18 04 05.183  & $-$34 28 37.39  & S/D \\
H 1-42         & 357.2$-$04.5 & 17 57 25.17  & $-$33 35 42.9  & ext \\
H 2-7          & 357.3+04.0 & 17 23 24.936  & $-$28 59 06.05  & ext \\
SB 50          & 357.3$-$06.5  & 18 06 08.301  & $-$34 33 30.72  & S/D \\
PPA1749-3216 & 357.5$-$02.4 & 17 49 37.82  & $-$32 16 27.9  & N/D \\
PPA1802-3350 & 357.5$-$05.5 & 18 02 23.8  & $-$33 50 48  & N/D \\
Pe 1-11        & 358.0$-$05.1 & 18 01 42.89  & $-$33 15 28.3  & N/D \\
M 3-8          & 358.2+04.2 & 17 24 52.152  & $-$28 05 54.61  & ext \\
Bl D           & 358.2$-$01.1 & 17 46 02.818  & $-$31 03 39.33  & N/D \\
SB 52          & 358.3$-$07.3  & 18 11 39.900  & $-$34 00 21.99  & N/D \\
JaSt 3         & 358.4+01.6  & 17 35 22.745  & $-$29 22 17.40 & N/D \\
NGC 6563       & 358.5$-$07.3 & 18 12 02.753  & $-$33 52 07.14  & ext \\
JaSt 4         & 358.6+01.7  & 17 35 37.47  & $-$29 13 17.7 & N/D \\
JaSt 58 & 358.6$-$01.1  & 17 46 52.20  & $-$30 37 42.8 & N/D \\
PHR1752-3116 & 358.7$-$02.5 & 17 52 36.5  & $-$31 16 27  & N/D \\
SB 53          & 358.7$-$05.1  & 18 03 28.532  & $-$32 37 26.46  & N/D \\
H 1-50         & 358.7$-$05.2 & 18 03 53.461  & $-$32 41 42.15  & N/D \\
JaSt 5         & 358.8+01.7  & 17 35 52.65  & $-$28 58 25.7 & N/D \\
Th 3-26        & 358.8+03.0 & 17 31 09.298  & $-$28 14 50.43  & ext \\
JaSt 9         & 359.0+01.1  & 17 38 45.91  & $-$29 09 01.6 & N/D \\
M 3-48         & 359.0$-$04.1 & 17 59 56.823  & $-$31 54 27.46  & ext \\
M 1-29         & 359.1$-$01.7 & 17 50 18.003  & $-$30 34 54.90  & ext \\
H 2-33         & 359.4$-$03.4 & 17 58 12.535  & $-$31 08 05.99 & ext \\
KnFs 3         & 359.7$-$04.4 & 18 02 52.931  & $-$31 23 58.49  & N/D \\
PPA1738-2800 & 359.9+01.8 & 17 38 11.8  & $-$28 00 07  & N/D \\
\end{longtable}
\end{landscape}
}% End \longtabL








